Calibrating the Rigged Lottery: Making All Tickets Reliable

Although sparse training has been successfully used in various resource-limited deep learning tasks to save memory, accelerate training, and reduce inference time, the reliability of the produced sparse models remains unexplored. Previous research has shown that deep neural networks tend to be over-confident, and we find that sparse training exacerbates this problem. Therefore, calibrating the sparse models is crucial for reliable prediction and decision-making. In this paper, we propose a new sparse training method to produce sparse models with improved confidence calibration. In contrast to previous research that uses only one mask to control the sparse topology, our method utilizes two masks, including a deterministic mask and a random mask. The former efficiently searches and activates important weights by exploiting the magnitude of weights and gradients. While the latter brings better exploration and finds more appropriate weight values by random updates. Theoretically, we prove our method can be viewed as a hierarchical variational approximation of a probabilistic deep Gaussian process. Extensive experiments on multiple datasets, model architectures, and sparsities show that our method reduces ECE values by up to 47.8\% and simultaneously maintains or even improves accuracy with only a slight increase in computation and storage burden.

==> sections/_s3_preliminaries.tex <==
\section{Preliminaries}


\subsection{Dropout}

Dropout is a widely-used method to overcome the over-fitting problem~\citep{hinton2012improving, wan2013regularization, srivastava2014dropout}, which can be viewed as a variational approximation to the probabilistic deep Gaussian process~\citep{gal2016dropout}. Unit dropout is a popular type of dropout that randomly discards units (neurons) at each training step. Weight dropout is another type, which randomly drops individual weights at each training step and is more flexible than unit dropout. Both methods only use dropout during training phase and remove them during testing.



In addition to removing dropout masks during testing, MC dropout collects multiple models by randomly sampling multiple dropout masks~\citep{gal2016dropout}. The predictions of these models are then averaged as the final predictions, which can approach the posterior better than weights and unit dropout and leads to higher performance~\citep{gal2016dropout}. In addition, it follows the paradigm of deep ensembles and can lead to improved confidence calibration properties~\citep{guo2017calibration, zhang2019confidence, roelofs2022mitigating}.
However, it requires additional forward FLOPs during testing and slows down the prediction speed. In addition, it collects multiple models with increasing sparsity, which can lead to a decrease in the accuracy of sparse training.


\subsection{Weight Averaging}

Weight Averaging is a new way of ensembling of neural networks~\citep{izmailov2018averaging, wortsman2022model}. Given multiple models, instead of averaging the output predictions of these models, this new ensemble approach averages the weights of these models. In this way, we still get one model at the end, which reduces the forward FLOPs and speeds up the prediction. In addition, when these models used for ensemble are located in a single low error basin, it usually leads to wider optima and better generalization. However, although previous ensemble methods based on prediction averaging can improve the confidence calibration of the model~\citep{guo2017calibration, roelofs2022mitigating}, weight averaging does not have the same effect~\citep{wortsman2022model}.


